Bridging Cache-Friendliness and Concurrency: A Locality-Optimized In-Memory B-Skiplist

Skiplists are widely used for in-memory indexing in many key-value stores, such as RocksDB and LevelDB, due to their ease of implementation and simple concurrency control mechanisms. However, traditional skiplists suffer from poor cache locality, as they store only a single element per node, leaving performance on the table. Minimizing last-level cache misses is key to maximizing in-memory index performance, making high cache locality essential. In this paper, we present a practical concurrent B-skiplist that enhances cache locality and performance while preserving the simplicity of traditional skiplist structures and concurrency control schemes. Our key contributions include a top-down, single-pass insertion algorithm for B-skiplists and a corresponding simple and efficient top-down concurrency control scheme. On 128 threads, the proposed concurrent B-skiplist achieves between 2x-9x higher throughput compared to state-of-the-art concurrent skiplist implementations, including Facebook's concurrent skiplist from Folly and the Java ConcurrentSkipListMap. Furthermore, we find that the B-skiplist achieves competitive (0.9x-1.7x) throughput on point workloads compared to state-of-the-art cache-optimized tree-based indices (e.g., Masstree). For a more complete picture of the performance, we also measure the latency of skiplist and tree-based indices and find that the B-skiplist achieves between 3.5x-103x lower 99% latency compared to other concurrent skiplists and between 0.85x-64x lower 99% latency compared to tree-based indices on point workloads with inserts.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> bskip-implementation.tex <==
\section{Fixed-size nodes in the \bskiplist}\label{sec:impl}

This section describes the proposed modification to the theoretical \bskiplist
structure of enforcing \emph{fixed-size nodes} and explains how this practical design
choice reduces data movement during insertions.  Furthermore, it shows
that this change does not affect the \bskiplist's theoretical bounds. Recall
that each node in a \bskiplist has a key array with $B$ elements, a RW lock, and
a \texttt{next} pointer. Internal nodes have an additional array of
\texttt{down} pointers.

\para{Structure} As mentioned in~\secref{intro}, due to the \bskiplist's
randomized structure, any practical \bskiplist implementation must handle the
case where the number of elements in a node exceeds some fixed-size array
allocation.  The number of keys that are supposed to be in a node may exceed a
fixed bound, depending on the sequence of coin flips. Given a \bskiplist with
$n$ elements and promotion probability $p = 1/B$, the expected number of
elements in a node is $\Theta(B)$, but the worst-case number of elements in a
given node is $\Theta(B\log n)$ w.h.p. Therefore, it is highly likely that there
will be nodes that exceed any fixed size $\Theta(B)$.

The naive solution of table doubling in nodes enables all keys meant for a node
to fit in the corresponding array, but leads to suboptimal performance of
insertions.  Suppose that there are $k$ elements stored contiguously in a
node. Inserting an element in that node requires $\Theta(k/Z)$ cache-line
transfers to maintain the elements in sorted order in that node because on
average, half of the elements must be shifted to the right to make room for the
new element. As mentioned in~\secreftwo{intro}{prelim}, w.h.p., there is a node
in the \bskiplist with $k = \Theta(B\log n)$ elements, so the worst-case
insertion cost in a \bskiplist is $\Theta(\log n)$ cache-line accesses w.h.p.

To alleviate this issue, we modify the \bskiplist design to require fixed-size
node allocations, which may potentially result in node \defn{overflow splits}
(i.e., node splits due to overflow) in addition to \defn{promotion splits} due
to randomization.  If nodes were allowed to grow arbitrarily large, the
worst-case number of elements moved (i.e., shifted to maintain sorted order)
during an insert is $\Theta(B\log n)$, which would take $\Theta(\log n)$ cache
misses. However, by requiring that the nodes have at most $B$ elements, the
number of element moves in any node is at most $B$. As mentioned
in~\secref{intro}, the choice of fixed-size nodes does not affect the
theoretical bounds, because a query would still have to perform $\Theta(\log n)$
cache-line transfers in the worst case w.h.p. However, minimizing the cost of
inserts is important for practical efficiency, as element moves must be linear
in the node size, while queries can skip over parts of the node e.g., via binary
search.

\brian{read this again, something feels not quite right}

% However,
% we focus on minimizing the cost of inserts (i.e., writes) because
% writes are more expensive than reads.

~\figref{fake-node-example} illustrates an example of a node resulting from an
overflow split. As shown in the diagram, the design choice of fixed-size nodes
relaxes the theoretical \bskiplist invariant that every header of a node has
been promoted to the next highest level. When a node becomes full, it splits
using the same procedure described in~\secref{prelim}. If node \texttt{x} is
full, half of its keys (and \texttt{down} pointers, if it is an internal node)
will be moved into a new node \texttt{y}. Next, the pointers will be adjusted
such that \texttt{y->next = x->next} and \texttt{x->next = y}. However, since
the split is not due to promotion, there is no corresponding key with a down
pointer to \texttt{y} in an upper level. However, node \texttt{y} is still
reachable via horizontal pointers from \texttt{x}.  As we shall see, fixed-size
nodes does not affect the \bskiplist's correctness or theoretical bounds.

\begin{figure}[t]
  \centering \includegraphics[width=\linewidth]{figs/fake-node-example.pdf}
  \caption{Example of a \bskiplist with fixed-size nodes ($B = 4$).  The blue
    node is the result of a overflow split, and the dotted
    box around two nodes represents one logical node (in theory).}
  \label{fig:fake-node-example}
\end{figure}

\para{Correctness and bounds} The nodes created from overflow splits do not
affect the correctness of inserts or searches, as operations in the \bskiplist
still follow a left-to-right and top-to-bottom traversal order. The elements in
these \defn{overflow split} nodes are still reachable from the top of the
\bskiplist through \texttt{next} pointers at their respective levels. The only
difference is that they are not reachable from \texttt{down} pointers from the
level above, which is not a necessary condition for valid searches. From the
point of view of the operation, the overflow nodes can be thought of one logical
node but just stored in different memory blocks and connected by pointers.

Next, we will show that the choice of fixing node sizes does not
affect the \bskiplist's theoretical guarantees.

\begin{lemma}
  A \bskiplist with fixed-size nodes of size $B = \Theta(Z)$ and with $n$
  elements supports finds and inserts in $\Theta(\log_Z n)$ cache-line transfers in
  expectation and $\Theta(\log n)$ cache-line transfers w.h.p.
\end{lemma}

\begin{proof}
The \bskiplist's
theoretical bounds depend on the expected number of elements between
each promotion and the expected height of the \bskiplist.

With a promotion
probability of $p = 1/B$, the expected number of tails before a head (i.e., the number of elements in any node) is
$\Theta(B)$.
As long as the node size $B = \Omega(Z)$, reading $k$ contiguous elements in one level of the \bskiplist takes $O(k/Z)$ cache-line transfers. Therefore, reading an expected $\Theta(B)$ elements at each level takes $\Theta(1)$ cache-line transfers in expectation.

Furthermore, the expected height remains $\Theta(\log_B n) = \Theta(\log_Z n)$, because the size of the list decreases by a factor of $B$ in each successive level in expectation. The number of levels until the list is size $\Theta(1)$ is $\Theta(\log_B n)$.

The proposed design of fixed-size nodes does not affect
the promotion probability and therefore the node size or the height of the \bskiplist, either in expectation or w.h.p. The only change is
that one logical node with an arbitrary-sized key array may be broken up
into several physical nodes with fixed-size key arrays. As long as the node size $B = \Omega(Z)$, the pointer indirections required to access the overflow nodes does
not asymptotically affect the count of the number of cache-line transfers in the
external-memory model.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> latexfigs/insert_find_table.tex <==
\begin{table*}[t]
\caption{\rev{Throughput (thr., in operations per second) and normalized performance of point operations in the
    \btree and \leafdstree.  Point operation throughput is reported in
    operations/s.  We use N.P. to denote the normalized performance in the
    \btree (\leafdstree) compared to the best \btree (\leafdstree) configuration
    for that operation (1.0 is the best possible value).}}
  \begin{center}
    \resizebox{.7\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{crrrrrrrrrrrr}
  \hline
  \multicolumn{5}{c}{\textit{\btree}}  &
                                         \multicolumn{7}{c}{\textit{\leafdstree}}
  \\
  \cmidrule(lr){1-5}   \cmidrule(lr){7-13}
 & \multicolumn{2}{c}{\textit{Insert}} &
   \multicolumn{2}{c}{\textit{Find}}  &&&& & \multicolumn{2}{c}{\textit{Insert}} &
   \multicolumn{2}{c}{\textit{Find}}  \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){10-11}   \cmidrule(lr){12-13}
 \begin{tabular}{@{}c@{}}\textit{Node size} \\ \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.}
  &&\begin{tabular}{@{}c@{}}\textit{Header size} \\
      \textit{(elts)}\end{tabular}&\begin{tabular}{@{}c@{}}\textit{Block size}
                                     \\
                                     \textit{(elts)}\end{tabular}&  \begin{tabular}{@{}c@{}}\textit{Total
                                                                      size} \\
                                                                      \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.}\\
  \hline
256&8.72E6&0.47&2.66E7&0.92&&4&4&384&1.05E7&0.54&2.96E7&0.94\\
512&1.56E7&0.84&2.81E7&0.97&&4&8&640&1.42E7&0.73&2.96E7&0.94\\
1024&1.86E7&1&2.86E7&0.98&&8&8&1280&1.63E7&0.84&3.05E7&0.96\\
2048&1.74E7&0.93&2.84E7&0.98&&8&16&2304&1.83E7&0.94&3.09E7&0.98\\
4096&1.34E7&0.72&2.91E7&1&&16&16&4608&1.87E7&0.97&3.16E7&1.00\\
8192&8.04E6&0.43&2.60E7&0.89&&16&32&8704&1.87E7&0.97&3.12E7&0.99\\
16384&4.27E6&0.23&1.59E7&0.55&&32&32&17408&1.94E7&1.00&3.02E7&0.96\\
32768&2.20E6&0.12&1.50E7&0.52&&32&64&33792&1.84E7&0.95&2.97E7&0.94\\
65536&1.12E6&0.06&1.40E7&0.48&&64&64&67584&1.73E7&0.89&1.73E7&0.55\\
  \hline
\end{tabular}
}
\label{tab:point-ops-all}
\end{center}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latexfigs/lock_table.tex <==

\begin{table}[t]
\centering

\begin{tabular}{@{}ccccc@{}}
 \hline
  & \multicolumn{2}{c}{B-tree} & \multicolumn{2}{c}{B-skiplist} \\
  Insert \% &  root lock & 99.9\% latency& root lock &  99.9\% latency \\
 \hline
 % took the numbers from ycsb sheet if they were there, else the uniform sheet
 1 & 415 & 4441 & 0 & 2083  \\
 5 & 1872 & 7724 & 1 & 2271 \\
 10 & 3533 & 10494 & 1 & 2261  \\
  25 & 5880 & 11571 & 2 & 2509 \\
  50 & 8377& 13285 & 3 & 2996 \\
 100 & 26070 & 17192 & 7& 5143  \\ [1ex]
 \hline
\end{tabular}
\caption{The number of times the write lock on the root is taken and the 99.9 percentile latency of operation on a workload of 100M
total find/insert operations with varying percentages of inserts. The B-tree
implements latch crabbing with optimistic concurrency control (OCC) and the B-skiplist implements
the proposed top-down concurrency control scheme. \brian{what percentage, at most these root locks account for .02\% of the operations, so maybe 99.9?}}
\label{tab:root-lock}
\end{table}

==> latexfigs/micros-table-old.tex <==
\begin{table*}[t]
  \begin{center}
 \resizebox{\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{@{}llllllllllllllllllllll@{}}
  \hline
  & & \multicolumn{8}{c}{\textit{100\% finds}}  & &
                                                    \multicolumn{8}{c}{\textit{100\%
                                                    inserts}} \\
  \cmidrule(lr){4-11}   \cmidrule(lr){13-20}
\textit{Bytes} & \textit {Elts} & \textit{$c$}
%  & \textit{TP} &  \begin{tabular}{@{}c@{}}\textit{Distance} \\ \textit{from
                      %                       best}\end{tabular}
  & \textit{TP} & \textit{DFB}
  & \textit{90\%} &  \textit{DFB}
  & \textit{99\%} &  \textit{DFB}
  & \textit{99.9\%} & \textit{DFB}
  & & \textit{TP} & \textit{DFB}
  & \textit{90\%} &  \textit{DFB}
  & \textit{99\%} &  \textit{DFB}
  & \textit{99.9\%} & \textit{DFB}
  \\
  \hline
  \iffalse
\multirow{3}{*}{512}&\multirow{3}{*}{32}&0.5&23.2&0.51&2.9E03&0.44&3.6E03&0.40&5.1E03&0.39&&12.1&0.43&4.7E03&0.50&1.4E04&0.23&2.8E05&0.02\\
&&1&40.9&0.90&1.5E03&0.87&1.7E03&0.85&2.2E03&0.88&&20.2&0.71&3.4E03&0.68&4.4E03&0.73&7.0E03&0.68\\
&&2&38.2&0.84&1.7E03&0.76&2.0E03&0.73&2.7E03&0.74&&14.0&0.49&5.2E03&0.45&1.1E04&0.30&2.1E04&0.23\\
  \hline
\multirow{3}{*}{1024}&\multirow{3}{*}{64}&0.5&44.5&0.98&1.3E03&0.97&1.5E03&0.96&2.1E03&0.96&&28.3&1.00&2.4E03&1.00&3.3E03&0.97&4.8E03&0.99\\
&&1&43.7&0.96&1.4E03&0.95&1.6E03&0.94&2.0E03&0.98&&22.5&0.80&2.9E03&0.82&5.1E03&0.63&1.1E04&0.45\\
&&2&38.7&0.85&1.6E03&0.78&1.9E03&0.77&2.5E03&0.79&&14.5&0.51&5.2E03&0.46&7.7E03&0.42&1.2E04&0.39\\
    \hline
\multirow{3}{*}{2048}&\multirow{3}{*}{128}&0.5&45.5&1.00&1.3E03&1.00&1.5E03&1.00&2.0E03&1.00&&27.9&0.99&2.4E03&1.00&3.2E03&1.00&5.1E03&0.93\\
 &&1&41.7&0.92&1.4E03&0.90&1.7E03&0.89&2.1E03&0.94&&22.1&0.78&3.0E03&0.78&4.1E03&0.78&6.4E03&0.75\\
 & &2&37.0&0.81&1.7E03&0.76&2.0E03&0.74&2.6E03&0.75&&13.5&0.48&5.5E03&0.43&9.5E03&0.34&1.5E04&0.31\\
    \hline
\multirow{3}{*}{4096}&\multirow{3}{*}{256}&0.5&39.3&0.86&1.5E03&0.84&1.8E03&0.83&2.4E03&0.82&&22.7&0.80&3.0E03&0.78&3.8E03&0.84&4.8E03&1.00\\
&&1&36.6&0.80&1.7E03&0.76&2.0E03&0.75&2.6E03&0.75&&19.1&0.67&3.6E03&0.65&5.0E03&0.64&7.5E03&0.64\\
&&2&31.8&0.70&2.0E03&0.63&2.4E03&0.62&3.4E03&0.59&&9.8&0.35&9.8E03&0.24&2.1E04&0.15&3.4E04&0.14\\
    \hline
\multirow{3}{*}{8192}&\multirow{3}{*}{512}&0.5&30.6&0.67&2.1E03&0.61&2.4E03&0.60&3.3E03&0.60&&15.6&0.55&4.5E03&0.53&5.5E03&0.59&6.5E03&0.74\\
&&1&25.9&0.57&2.6E03&0.50&3.0E03&0.50&3.9E03&0.51&&12.6&0.44&5.6E03&0.42&9.3E03&0.35&1.4E04&0.33\\
&&2&26.1&0.57&2.6E03&0.50&3.0E03&0.49&4.0E03&0.50&&10.8&0.38&7.2E03&0.33&1.3E04&0.25&1.8E04&0.26\\

  \fi
  &&0.5&23.2&0.5&2.9E3&0.4&3.6E3&0.4&5.1E3&0.4&&12.1&0.4&4.7E3&0.5&1.4E4&0.2&2.8E5&0.0\\
  512&32&1&40.9&0.9&1.5E3&0.9&1.7E3&0.9&2.2E3&0.9&&20.2&0.7&3.4E3&0.7&4.4E3&0.7&7.0E3&0.7\\
  &&2&38.2&0.8&1.7E3&0.8&2.0E3&0.7&2.7E3&0.7&&14.0&0.5&5.2E3&0.5&1.1E4&0.3&2.1E4&0.2\\
  \hline
  &&0.5&\textbf{44.5}&\textbf{1.0}&\textbf{1.3E3}&\textbf{1.0}&\textbf{1.5E3}&\textbf{1.0}&\textbf{2.1E3}&\textbf{1.0}&&\textbf{28.3}&\textbf{1.0}&\textbf{2.4E3}&\textbf{1.0}&\textbf{3.3E3}&\textbf{1.0}&\textbf{4.8E3}&\textbf{1.0}&\\
  1024&64&1&\textbf{43.7}&\textbf{1.0}&1.4E3&0.9&1.6E3&0.9&\textbf{2.0E3}&\textbf{1.0}&&22.5&0.8&2.9E3&0.8&5.1E3&0.6&1.1E4&0.5\\
  &&2&38.7&0.9&1.6E3&0.8&1.9E3&0.8&2.5E3&0.8&&14.5&0.5&5.2E3&0.5&7.7E3&0.4&1.2E4&0.4\\
  \hline
  &&0.5&\textbf{45.5}&\textbf{1.0}&\textbf{1.3E3}&\textbf{1.0}&\textbf{1.5E3}&\textbf{1.0}&\textbf{2.0E3}&\textbf{1.0}&&\textbf{27.9}&\textbf{1.0}&\textbf{2.4E3}&\textbf{1.0}&\textbf{3.2E3}&\textbf{1.0}&5.1E3&0.9\\
  2048&128&1&41.7&0.9&1.4E3&0.9&1.7E3&0.9&2.1E3&0.9&&22.1&0.8&3.0E3&0.8&4.1E3&0.8&6.4E3&0.8\\
  &&2&37.0&0.8&1.7E3&0.8&2.0E3&0.7&2.6E3&0.8&&13.5&0.5&5.5E3&0.4&9.5E3&0.3&1.5E4&0.3\\
  \hline
  &&0.5&39.3&0.9&1.5E3&0.8&1.8E3&0.8&2.4E3&0.8&&22.7&0.8&3.0E3&0.8&3.8E3&0.8&\textbf{4.8E3}&\textbf{1.0}&\\
  4096&256&1&36.6&0.8&1.7E3&0.8&2.0E3&0.7&2.6E3&0.8&&19.1&0.7&3.6E3&0.6&5.0E3&0.6&7.5E3&0.6\\
  &&2&31.8&0.7&2.0E3&0.6&2.4E3&0.6&3.4E3&0.6&&9.8&0.3&9.8E3&0.2&2.1E4&0.2&3.4E4&0.1\\
  \hline
  &&0.5&30.6&0.7&2.1E3&0.6&2.4E3&0.6&3.3E3&0.6&&15.6&0.6&4.5E3&0.5&5.5E3&0.6&6.5E3&0.7\\
  8192&512&1&25.9&0.6&2.6E3&0.5&3.0E3&0.5&3.9E3&0.5&&12.6&0.4&5.6E3&0.4&9.3E3&0.3&1.4E4&0.3\\
  &&2&26.1&0.6&2.6E3&0.5&3.0E3&0.5&4.0E3&0.5&&10.8&0.4&7.2E3&0.3&1.3E4&0.2&1.8E4&0.3\\
  \hline
\end{tabular}
}
\end{center}
\caption{\todo{microbenchmarks on unif random. TP = throughput (in ops/s). 90\%, 99\%, 99.9\% are in
    us. DFB = distance from best (1.0 is the best, all others are
    normalized). on uniform random workload. $p = 1/(c \times elts)$.}}
    \label{tab:micros}
%    $p = 1/(\gamma \times (B/2\times\texttt{sizeof(T)}))$.}}
\end{table*}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latexfigs/range-tables.tex <==
\begin{table*}[t]
\caption{\rev{Throughput (thr., in expected elements per second) of range
  queries of varying maximum lengths (\texttt{max\_len}) in the
  \btree and \leafdstree. We also report the normalized
  performance (N.P.) compared to the best-case performance for each operation
  (up to 1.0).}}
  \begin{center}
    \resizebox{\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{crrrrrrrrrrrrrrrrrrrrr}
  \hline
  \multicolumn{9}{c}{\textit{\btree}}  &
                                         \multicolumn{12}{c}{\textit{\leafdstree}} \\
 \cmidrule(lr){1-9}  \cmidrule(lr){10-21}  \\
& \multicolumn{4}{c}{\textit{Short} (\texttt{max\_len} = 100)} &
                                       \multicolumn{4}{c}{\textit{Long}
                                                                 (\texttt{max\_len}
                                                                 = 100,000)} &&&&&
                                                                                \multicolumn{4}{c}{\textit{Short}
                                                                                (\texttt{max\_len} = 100)} &
                                       \multicolumn{4}{c}{\textit{Long} (\texttt{max\_len} = 100,000)}   \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}   \cmidrule(lr){14-17} \cmidrule(lr){18-21} \\
 & \multicolumn{2}{c}{\textit{Map}} &
   \multicolumn{2}{c}{\textit{Iterate}}  & \multicolumn{2}{c}{\textit{Map}} &
   \multicolumn{2}{c}{\textit{Iterate}}   &&&& & \multicolumn{2}{c}{\textit{Map}} &
   \multicolumn{2}{c}{\textit{Iterate}} & \multicolumn{2}{c}{\textit{Map}} &
   \multicolumn{2}{c}{\textit{Iterate}}  \\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-9}
  \cmidrule(lr){14-15}  \cmidrule(lr){16-17}  \cmidrule(lr){18-19}  \cmidrule(lr){20-21}
 \begin{tabular}{@{}c@{}}\textit{Node size} \\ \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.} & \textit{Thr.} & \textit{N.P.}
 & \textit{Thr.} & \textit{N.P.} &&\begin{tabular}{@{}c@{}}\textit{Header size} \\
      \textit{(elts)}\end{tabular}&\begin{tabular}{@{}c@{}}\textit{Block size}
                                     \\
                                     \textit{(elts)}\end{tabular}&  \begin{tabular}{@{}c@{}}\textit{Total
                                                                      size} \\
                                                                      \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.}&
\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.}\\
  \hline
  256&8.56E8&0.77&9.48E8&0.72&1.88E9&0.25&2.16E9&0.29&&4&4&384&4.76E8&0.53&7.15E8&0.59&7.32E8&0.14&1.20E9&0.22\\
512&9.58E8&0.86&1.05E9&0.80&2.12E9&0.28&2.43E9&0.32&&4&8&640&6.86E8&0.76&8.93E8&0.73&1.32E9&0.25&1.71E9&0.32\\
1024&1.01E9&0.91&1.13E9&0.85&2.69E9&0.36&3.13E9&0.42&&8&8&1280&7.91E8&0.88&9.45E8&0.78&1.72E9&0.32&1.85E9&0.35\\
2048&1.08E9&0.97&1.20E9&0.91&4.23E9&0.56&4.51E9&0.60&&8&16&2304&8.98E8&1.00&1.07E9&0.88&2.46E9&0.46&2.54E9&0.47\\
4096&1.11E9&1.00&1.26E9&0.95&5.18E9&0.69&5.33E9&0.71&&16&16&4608&8.99E8&1.00&1.13E9&0.93&3.17E9&0.59&3.22E9&0.60\\
8192&1.10E9&0.99&1.28E9&0.97&5.97E9&0.80&6.36E9&0.85&&16&32&8704&8.86E8&0.99&1.22E9&1.00&4.19E9&0.78&4.25E9&0.79\\
16384&1.08E9&0.98&1.29E9&0.98&6.60E9&0.88&7.00E9&0.93&&32&32&17408&8.14E8&0.91&1.17E9&0.96&4.75E9&0.89&4.75E9&0.89\\
32768&1.08E9&0.97&1.30E9&0.98&7.18E9&0.96&7.36E9&0.98&&32&64&33792&6.73E8&0.75&1.05E9&0.87&5.21E9&0.97&5.16E9&0.96\\
65536&1.09E9&0.98&1.32E9&1.00&7.50E9&1.00&7.49E9&1.00&&64&64&67584&5.74E8&0.64&9.83E8&0.81&5.35E9&1.00&5.35E9&1.00\\
  \hline
\end{tabular}
}
\label{tab:range-ops-all}
\end{center}
\end{table*}

\iffalse

\begin{table*}[t]
  \begin{center}
        \resizebox{.8\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{crrrrrrrrrrrrrrrr}
  \hline
 & \multicolumn{4}{c}{\textit{\texttt{max\_len} = 100}}  & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                  = 1,000}} & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                  = 10,000}} & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                               = 100,000}} \\
   & \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}}  &
                                                                                 \multicolumn{2}{c}{\textit{Map}}
                                                             &
                                                               \multicolumn{2}{c}{\textit{Iterate}} & \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}} &  \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}}  \\
  \cmidrule(lr){2-5}  \cmidrule(lr){6-9}   \cmidrule(lr){10-13}   \cmidrule(lr){14-17}
 \begin{tabular}{@{}c@{}}\textit{Node size} \\ \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}&\textit{Thr.} & \textit{N.P.}
  &\textit{Thr.} & \textit{N.P.}&\textit{Thr.}& \textit{N.P.}
                                                                &\textit{Thr.} &
                                                                              \textit{N.P.}&
                                                                                           \textit{Thr.} & \textit{N.P.}  &\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.} \\
  \hline

  \hline
\end{tabular}
}
\caption{\rev{Throughput (thr., in expected elements per second) of range
  queries of varying maximum lengths (\texttt{max\_len}) in the
  \btree. We also report the normalized
  performance (N.P.) compared to the best-case performance for each operation
  (up to 1.0).}}
\label{tab:plain-range}
\end{center}
\end{table*}

\begin{table*}[t]
  \begin{center}
        \resizebox{.8\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{cccrrrrrrrrrrrrrrrr}
  \hline
 & &&\multicolumn{4}{c}{\textit{\texttt{max\_len} = 100}}  & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                  = 1,000}} & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                  = 10,000}} & \multicolumn{4}{c}{\textit{\texttt{max\_len}
                                                               = 100,000}} \\
   &&& \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}}  &
                                                                                 \multicolumn{2}{c}{\textit{Map}}
                                                             &
                                                               \multicolumn{2}{c}{\textit{Iterate}} & \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}} &  \multicolumn{2}{c}{\textit{Map}}  & \multicolumn{2}{c}{\textit{Iterate}}  \\
  \cmidrule(lr){4-7} \cmidrule(lr){8-11}   \cmidrule(lr){12-15}   \cmidrule(lr){16-19}
\begin{tabular}{@{}c@{}}\textit{Header} \\
      \textit{(elts)}\end{tabular}&\begin{tabular}{@{}c@{}}\textit{Block}
                                     \\
                                     \textit{(elts)}\end{tabular}&  \begin{tabular}{@{}c@{}}\textit{Total
                                                                      } \\
                                                                      \textit{(bytes)}\end{tabular}&
\textit{Thr.} & \textit{N.P.}&\textit{Thr.} & \textit{N.P.}
  &\textit{Thr.} & \textit{N.P.}&\textit{Thr.}& \textit{N.P.}
                                                                &\textit{Thr.} &
                                                                              \textit{N.P.}&
                                                                                           \textit{Thr.} & \textit{N.P.}  &\textit{Thr.} & \textit{N.P.}& \textit{Thr.} & \textit{N.P.} \\
  \hline
4&4&384&4.76E8&0.53&7.15E8&0.59&6.86E8&0.22&1.12E9&0.30&7.25E8&0.15&1.19E9&0.23&7.32E8&0.14&1.20E9&0.22\\
4&8&640&6.86E8&0.76&8.93E8&0.73&1.19E9&0.38&1.56E9&0.42&1.31E9&0.26&1.69E9&0.33&1.32E9&0.25&1.71E9&0.32\\
8&8&1280&7.91E8&0.88&9.45E8&0.78&1.53E9&0.49&1.70E9&0.46&1.70E9&0.34&1.84E9&0.36&1.72E9&0.32&1.85E9&0.35\\
8&16&2304&8.98E8&1.00&1.07E9&0.88&2.16E9&0.69&2.28E9&0.61&2.42E9&0.49&2.51E9&0.49&2.46E9&0.46&2.54E9&0.47\\
16&16&4608&8.99E8&1.00&1.13E9&0.93&2.55E9&0.82&2.74E9&0.74&3.10E9&0.63&3.17E9&0.62&3.17E9&0.59&3.22E9&0.60\\
16&32&8704&8.86E8&0.99&1.22E9&1.00&3.00E9&0.96&3.32E9&0.89&4.04E9&0.82&4.14E9&0.81&4.19E9&0.78&4.25E9&0.79\\
32&32&17408&8.14E8&0.91&1.17E9&0.96&3.11E9&1.00&3.47E9&0.93&4.50E9&0.91&4.58E9&0.90&4.75E9&0.89&4.75E9&0.89\\
32&64&33792&6.73E8&0.75&1.05E9&0.87&3.04E9&0.98&3.72E9&1.00&4.86E9&0.98&4.96E9&0.97&5.21E9&0.97&5.16E9&0.96\\
64&64&67584&5.74E8&0.64&9.83E8&0.81&2.92E9&0.94&3.63E9&0.98&4.94E9&1.00&5.12E9&1.00&5.35E9&1.00&5.35E9&1.00\\
  \hline
\end{tabular}
}
\caption{\rev{Throughput (thr., in expected elements per second) of range
  queries of varying maximum lengths (\texttt{max\_len}) in the
  \leafdstree. We also report the normalized
  performance (N.P.) compared to the best-case performance for each operation
  (up to 1.0).}}
\label{tab:leafds-range}
\end{center}
\end{table*}
\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latexfigs/range_query_by_len.tex <==


\begin{figure}
  \centering
  \begin{tikzpicture}
    \begin{axis}[cycle list name=mylist,
         width=8cm, height=5cm,
        legend pos=north west,
        ylabel={Throughput (expected elts/s)},
                xlabel={Maximum query length},
        xtick=data,
        % bar width=5pt,
        legend columns=2,
        legend style ={font=\small},
        extra y ticks=1,
        enlarge x limits=0.12,
        xmode=log,
        log basis x={10},
        ymax = 7E9,
        % bar width=4pt,
      ]

   % \foreach \a in {Unsorted baseline, Sorted baseline, Unsorted bigleaf, Sorted bigleaf, Unsorted LeafDS, Sorted LeafDS}{
  % \foreach \a in {Map baseline, Iterate baseline, Map LeafDS, Iterate LeafDS,
  %   Map array, Iterate array}{
  \foreach \a in {Iterate B-tree, Map B-tree,  Iterate BP-tree, Map BP-tree}{
      \addplot table [
            discard if not={type}{\a},
          x=range query len, y expr=(\thisrow{throughput}), col sep=tab
        ] {tsvs/range_query_lens.tsv};

            \expandafter\addlegendentry\expandafter{\a}
    }
    \end{axis}
  \end{tikzpicture}
  \caption{Range operation thorughput as a function of the maximum length of each query.\footnotemark{}
     % \helen{do we want to keep the array as the ideal? i removed it for now}}
  \label{fig:range_queries_by_len}
\end{figure}

\footnotetext{The difference in performance between map and iterate in an already sorted B-tree comes from minor differences in their api, a map is specified by a start and an end, while iteration is specified by start and the number of elements.  This leads to different compiler optimizations around unrolling with how it handles comparisons and increments.  This was done to be able to compare with existing benchmarks and results in slightly different code in seemingly the same experiment.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latexfigs/ycsb_tables_old.tex <==

\begin{table}[t]
\centering
\begin{tabular}{@{}ll@{}}
 \hline
Workload & Description \\
 \hline
Load & 100\% inserts from empty\\
A&50\% finds, 50\% inserts \\
B&95\% finds, 5\% inserts \\
C&100\% finds  \\
E&95\% short range iterations (\maxlen = 100), 5\% inserts\ \\
% X&99.9\% finds, 0.1\% inserts \\
%Y&100\% inserts \\ [1ex]
 \hline
\end{tabular}
\caption{YCSB workload descriptions.}
\label{tab:ycsb-workloads}
\end{table}

\begin{table*}[t]
  \begin{center}
 \resizebox{\textwidth}{!}{
%\begin{tabular}{ccccccccccccccccccc}
\begin{tabular}{@{}llllllllllllllllllllllllll@{}}
  \hline
  % & & \multicolumn{7}{c}{\textit{Uniform}}  & & \multicolumn{7}{c}{\textit{Zipfian}} \\
 % \cmidrule(lr){3-9}   \cmidrule(lr){11-17}
  \textit{Metric} &  \textit{Workload} & \textit{\bskiplistshort} & \textit{\javashort}
&   \textit{\javashort/\bskiplistshort} & \textit{\btreeshort} & \textit{\btreeshort/\bskiplistshort} & \textit{\masstreeshort}
  & \textit{\masstreeshort/\bskiplistshort} &&
  \textit{\bskiplistshort} & \textit{\javashort}
&   \textit{\javashort/\bskiplistshort} & \textit{\btreeshort} & \textit{\btreeshort/\bskiplistshort} & \textit{\masstreeshort}
  & \textit{\masstreeshort/\bskiplistshort} \\%\textit{\openbwshort}
      \hline
        \multirow{5}{*}{TP}
        & Load\\
        & A \\
        & B \\
        & C \\  & E \\
        \hline
        & Load\\
        & A \\
        50\%  & B \\ 
        & C \\  
        & E \\
        \hline
        & Load\\
        & A \\
        90\%  & B \\ 
        & C \\  
        & E \\
        \hline
        & Load\\
        & A \\
        99\%  & B \\ 
        & C \\  
        & E \\
        \hline
\end{tabular}
}
\label{tab:ycsb-unif}
\end{center}
\caption{Throughput (in operations/s) \todo{and latencies} of the \bskiplist (\bskiplistshort), Java
  \skiplist (\javashort), optimistic \btree
  (\btreeshort), and \masstree (\masstreeshort) on
  uniform random workloads from YCSB. A number above 1 means that the system achieved higher throughput than the \bskiplist. \todo{add another one with zipf}\todo{also,
  maybe one of each of these for 90\%, 99\%, 99.9\%?}}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

==> tsvs/skiplist_uniform.tex <==
Workload	bskip	bskip ratio	btree	btree ratio	java skip	java skip ratio	masstree	masstree ratio	proactice btree	proactive btree ratio
load	30.66	1	22.20	0.7239500123	6.09	0.1986088445	13.7874	0.4496386836	15.8329	0.5163471222
A	35.05	1	35.66	1.017289486	6.28	0.1791700955	28.8021	0.8217316892	21.0043	0.5992583499
B	44.35	1	50.62	1.141347667	7.86	0.1772325449	45.0374	1.015533463	34.0994	0.7688961123
C	45.52	1	53.42	1.173651705	9.73	0.2137735507	47.5945	1.045677827	38.2189	0.8396906431
E	30.0	1	43.6	1.454367303			3.6117	0.1203776372		

==> tsvs/skiplist_zipfian.tex <==
Workload	bskip	bskip ratio	btree	btree ratio	java skip	java skip ratio	masstree	masstree ratio	proactice btree	proactive btree ratio
load	30.66	1	22.20	0.7239500123	6.09	0.1986088445	13.7874	0.4496386836	15.8329	0.5163471222
A	35.05	1	35.66	1.017289486	6.28	0.1791700955	28.8021	0.8217316892	21.0043	0.5992583499
B	44.35	1	50.62	1.141347667	7.86	0.1772325449	45.0374	1.015533463	34.0994	0.7688961123
C	45.52	1	53.42	1.173651705	9.73	0.2137735507	47.5945	1.045677827	38.2189	0.8396906431
E	30.0	1	43.6	1.454367303			3.6117	0.1203776372		
